Proactive Posturing of Large Power Grid for Mitigating Hurricane Impacts

In the past decade, natural disasters such as hurricanes have challenged the operation and control of U.S. power grid. It is crucial to develop proactive strategies to assist grid operators for better emergency response and minimized electricity service interruptions; the better the grid may be preserved, the faster the grid can be restored. In this paper, we propose a proactive posturing of power system elements, and formulate a Security-Constrained Optimal Power Flow (SCOPF) informed by cross-domain hurricane modeling as well as its potential impacts on grid elements. Simulation results based on real-world power grid and historical hurricane event have verified the applicability of the proposed optimization formulation, which shows potential to enable grid operators and planners with interactive cross-domain data analytics for mitigating hurricane impacts.

==> IEEE Conference Template - Short Version (RR11012021)/Nomenclature.tex <==
\addcontentsline{toc}{section}{Nomenclature}
\noindent
\textbf{Indices and Sets:}
\begin{IEEEdescription}[\IEEEusemathlabelsep\IEEEsetlabelwidth{${p}_{tgc}^{\mathrm{max}},{p}_{tgc}^{\mathrm{min}}$}]
    \item[$\mathcal{T}$] {Set of discrete time slots, with index $t$.}
    \item[$\Gcal$] {Set of all generators.}
	\item[$\Gcal_{t}$] {Set of all generators available at time $t\in \Tcal$.}
	\item[$\Ccal_{t}$] {Set of all contingency cases with $0\in\Ccal_{t}$ representing the base case (normal operation).}
	\item[$\Gcal_{tc}$] {Set of all generators that are available at time $t\in\Tcal$ and contingency $c\in\Ccal_{t}$, such that
		\begin{align}
			\Gcal_{t}=\cup_{c\in\Ccal_{t}}\Gcal_{tc}.\nonumber
		\end{align}}
	 \item[$\Vcal$] {Set of network buses.}
    \item[$\Ecal_{tc}$] {Set of lines at time $t\in \Tcal$ and contingency $c\in\Ccal_{t}$, such that
        \begin{align}
			\Ecal_{tc}=\Vcal \times \Vcal.\nonumber
		\end{align}}
\end{IEEEdescription}
\textbf{Parameters:}
\begin{IEEEdescription}[\IEEEusemathlabelsep\IEEEsetlabelwidth{${p}_{tgc}^{\mathrm{max}},{p}_{tgc}^{\mathrm{min}}$}]
	\item[$\alpha^{\mathrm{sqr}}_{tg}$]{Coefficient of quadratic term in cost function at time $t$ by unit $g\in\Gcal_{t}$.}
	\item[$\alpha^{\mathrm{lin}}_{tg}$]{Coefficient of linear term in cost function at time $t$ by unit $g\in\Gcal_{t}$.}
	\item[$\zeta_{tg}$]{Fixed cost coefficient at time $t$ by unit $g\in\Gcal_{t}$.}
	\item[$\eta_{tg}^{+},\eta_{tg}^{-}$]{Contingency reserves cost coefficients at time $t$ by unit $g\in\Gcal_{t}$.}
	\item[$\mu_{tg}^{+}, \mu_{tg}^{-}$]{Load-following ramping reserve cost coefficients at time $t$ by unit $g\in\Gcal_{t}$.}
	\item[$\beta_{tg}^{+}, \beta_{tg}^{-}$]{Active power re-dispatch cost coefficients at time $t$ by unit $g\in\Gcal_{t}$.}
	\item[$\kappa_{g}$]{Ramp wear and tear cost coefficients at time $t$ by unit $g\in\Gcal_{t}$.}
	\item[${p}_{tgc}^{\mathrm{max}},{p}_{tgc}^{\mathrm{min}}$] {Upper/lower limits on active power injections.}
	\item[${r}_{tg}^{\mathrm{max}},{r}_{tg}^{\mathrm{min}}$] {Upper/lower limits on reserve capacity in post-contingency dispatch quantities.}
	\item[${w}_{tg}^{\mathrm{max}},{w}_{tg}^{\mathrm{min}}$] {Upper/Lower limits on load-following reserve quantities.}
	\item[$\Delta_{g}^{\mathrm{max}},\Delta_{g}^{\mathrm{min}}$] {Upper/lower limits on transitions from base to post-contigency cases.}
	\item[$\psi_{tsc}$] {Conditional probability of contingency at time $t\in\Tcal$ and contingency $c\in\Ccal_{t}$.}
	\item[$\gamma_{t}$] {Probability of transitioning to period $t\in\Tcal$ without branching off from the central base case path to a contingency.}
\end{IEEEdescription}
\textbf{Variables:}
\begin{IEEEdescription}[\IEEEusemathlabelsep\IEEEsetlabelwidth{${p}_{tgc}^{\mathrm{max}},{p}_{tgc}^{\mathrm{min}}$}]
	\item[$p_{tgc}$] {Active power injection at time $t\in\Tcal$ by unit $g\in\Gcal_{t}$and contingency $c\in\Ccal_{t}$.}
	\item[$p^{\mathrm{ref}}_{tg}$] {Reference active power value from which generation variations are defined.}
	\item[$r^{+}_{tg},r^{-}_{tg}$] {Upward and downward contingency reserve quantities at time $t$ by unit $g\in\Gcal_{t}$.}
	\item[$w_{tg}^{+},w_{tg}^{-}$] {Upward and downward load-following ramping reserve quantities at time $t$ by unit $g\in\Gcal_{t}$.}
\end{IEEEdescription}



==> IEEE Conference Template - Short Version (RR11012021)/Notation.tex <==
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{amsthm}
\usepackage{amsfonts}
\usepackage{hyphenat}
\usepackage{hyperref}
\usepackage{times}
\usepackage{psfrag}
\usepackage{ifpdf}
\usepackage{array}
\usepackage{multirow}
\usepackage{setspace}
\usepackage{latexsym}
\usepackage{enumerate}
\usepackage{mathtools}
\usepackage{float}
\usepackage{scalerel}
\usepackage{cite}
\usepackage{cleveref}
\usepackage{graphicx}
\usepackage{caption}
\usepackage{epstopdf}
%\usepackage[table]{xcolor}
\usepackage{subfig}
\usepackage{accents}
\usepackage{algorithm}
\usepackage{algorithmic} 
\usepackage{mathrsfs}
\usepackage{tabularx}
\usepackage{tikz}
\usepackage{pgfplots}
\usepackage{url}  %Required
\usepackage{caption}
\usepackage{rotating}


\newcommand{\sm}[2]{\scaleto{#1\mathstrut}{#2pt}}
%\newcommand{\ubar}[1]{\underaccent{\bar}{#1}}
\newcommand{\msh}{\!\!\:}
\newcommand{\nsh}{\!\!\!\:\:}
\definecolor{Fcolor}{rgb}{0,0.5,0.25}
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}

\newtheorem{theorem}{Theorem}
\newtheorem{definition}{Definition}
\newtheorem{lemma}{Lemma}
\newtheorem{corollary}{Corollary}
\newtheorem{remark}{Remark}
\newtheorem{notation}{Notation}
\newtheorem{proposition}{Proposition}
\theoremstyle{definition}
\newtheorem{example}{Example}

\crefrangelabelformat{equation}{(#3#1#4)\,--\,(#5#2#6)}
\crefmultiformat{equation}{(#2#1#3)}{\,--\,(#2#1#3)}{#2#1#3}{#2#1#3}

\crefname{equation}{}{}
\crefname{figure}{Figure}{Figures}
\crefname{algorithm}{Algorithm}{Algorithms}
\crefname{table}{Table}{Tables}
\crefname{lemma}{Lemma}{Lemmas}
\crefname{theorem}{Theorem}{Theorems}
\crefname{remark}{Remark}{Remarks}
\crefname{section}{Section}{Sections}
\crefname{subsection}{Subsection}{Subsections}
\crefname{definition}{Definition}{Definitions}
%\oddsidemargin  0.0in
%\evensidemargin 0.0in
%\textwidth      6.50in
%\topmargin      -0.45in
%\textheight     9.0in


%\newcommand{\st}{\mathrm{subject~to}}
\newcommand{\tr}{\mathrm{tr}}
\newcommand{\onebf}{\boldsymbol{1}}

\newcommand{\T}{^{\!\top}}
\newcommand{\Tp}{^{\!\phantom{\top}}}

\newcommand{\la}{\langle}
\newcommand{\ra}{\rangle}


\newcommand{\asf}{\mathsf{a}}
\newcommand{\abf}{\boldsymbol{a}}
\newcommand{\Asf}{\boldsymbol{\mathsf{A}}}
\newcommand{\Abf}{\boldsymbol{A}}
\newcommand{\Acal}{\mathcal{A}}

\newcommand{\bsf}{\boldsymbol{\mathsf{b}}}
\newcommand{\bbf}{\boldsymbol{b}}
\newcommand{\Bsf}{\boldsymbol{\mathsf{B}}}
\newcommand{\Bbf}{\boldsymbol{B}}
\newcommand{\Bcal}{\mathcal{B}}
\newcommand{\Brm}{\mathrm{B}}
\newcommand{\Bch}{\check{\Bcal}}
\newcommand{\Bst}{\accentset{\ast}{\Bcal}}

\newcommand{\Csf}{\boldsymbol{\mathsf{C}}}
\newcommand{\Cbf}{\boldsymbol{C}}
\newcommand{\cbf}{\boldsymbol{c}}
\newcommand{\Ccal}{\mathcal{C}}
\newcommand{\Cbb}{\mathbb{C}}

\newcommand{\Dsf}{\boldsymbol{\mathsf{D}}}
\newcommand{\dbf}{\boldsymbol{d}}
\newcommand{\Dbf}{\boldsymbol{D}}
\newcommand{\Dcal}{\mathcal{D}}

\newcommand{\ebf}{\boldsymbol{e}}
\newcommand{\Ebf}{\boldsymbol{E}}
\newcommand{\Ecal}{\mathcal{E}}
\newcommand{\Erm}{\mathrm{E}}

\newcommand{\fbf}{\boldsymbol{f}}
\newcommand{\Fbf}{\boldsymbol{F}}
\newcommand{\Fcal}{\mathcal{F}}
\newcommand{\Frm}{\mathrm{F}}
\newcommand{\frm}{\mathrm{f}}
\newcommand{\Fch}{\check{\mathcal{F}}}

\newcommand{\gbf}{\boldsymbol{g}}
\newcommand{\Gbf}{\boldsymbol{G}}
\newcommand{\Gcal}{\mathcal{G}}

\newcommand{\hbf}{\boldsymbol{h}}
\newcommand{\Hbf}{\boldsymbol{H}}
\newcommand{\Hcal}{\mathcal{H}}
\newcommand{\Hbb}{\mathbb{H}}

\newcommand{\ibf}{\boldsymbol{i}}
\newcommand{\Ibf}{\boldsymbol{I}}
\newcommand{\irm}{\mathrm{i}}
\newcommand{\Irm}{\mathrm{I}}
\newcommand{\Ical}{\mathcal{I}}
\newcommand{\Ich}{\check{\Ical}}
\newcommand{\Ist}{\accentset{\ast}{\Ical}}

\newcommand{\jbf}{\boldsymbol{j}}
\newcommand{\Jbf}{\boldsymbol{J}}
\newcommand{\Jcal}{\mathcal{J}}

\newcommand{\Ksf}{\boldsymbol{\mathsf{K}}}
\newcommand{\kbf}{\boldsymbol{k}}
\newcommand{\Kbf}{\boldsymbol{K}}
\newcommand{\Kcal}{\mathcal{K}}
\newcommand{\Krm}{\mathrm{K}}

\newcommand{\lsf}{\mathsf{l}}
\newcommand{\lbf}{\boldsymbol{l}}
\newcommand{\Lbf}{\boldsymbol{L}}
\newcommand{\Lcal}{\mathcal{L}}

\newcommand{\msf}{\mathsf{m}}
\newcommand{\mbf}{\boldsymbol{m}}
\newcommand{\Mbf}{\boldsymbol{M}}
\newcommand{\mrm}{\mathrm{m}}
\newcommand{\Mcal}{\mathcal{M}}

\newcommand{\nrm}{\mathrm{n}}
\newcommand{\nbf}{\boldsymbol{n}}
\newcommand{\Nbf}{\boldsymbol{N}}
\newcommand{\Ncal}{\mathcal{N}}

\newcommand{\Ob}{\boldsymbol{O}}
\newcommand{\obf}{\boldsymbol{o}}

\newcommand{\pbf}{\boldsymbol{p}}
\newcommand{\Pbf}{\boldsymbol{P}}
\newcommand{\Pcal}{\mathcal{P}}

\newcommand{\qbf}{\boldsymbol{q}}
\newcommand{\Qbf}{\boldsymbol{Q}}
\newcommand{\Qcal}{\mathcal{Q}}
\newcommand{\qch}{\check{q}}

\newcommand{\rbf}{\boldsymbol{r}}
\newcommand{\Rbf}{\boldsymbol{R}}
\newcommand{\rrm}{\mathrm{r}}
\newcommand{\Rbb}{\mathbb{R}}
\newcommand{\Rcal}{\mathcal{R}}

\newcommand{\sbf}{\boldsymbol{s}}
\newcommand{\Sbf}{\boldsymbol{S}}
\newcommand{\Sbb}{\mathbb{S}}
\newcommand{\Scal}{\mathcal{S}}
\newcommand{\Srm}{\mathrm{S}}

\newcommand{\tsf}{\mathsf{t}}
\newcommand{\tbf}{\boldsymbol{t}}
\newcommand{\Tbf}{\boldsymbol{T}}
\newcommand{\trm}{\mathrm{t}}
\newcommand{\Tcal}{\mathcal{T}}

\newcommand{\usf}{\boldsymbol{\mathsf{u}}}
\newcommand{\ubf}{\boldsymbol{u}}
\newcommand{\Ubf}{\boldsymbol{U}}
\newcommand{\Usf}{\boldsymbol{\mathsf{U}}}

\newcommand{\vsf}{\boldsymbol{\mathsf{v}}}
\newcommand{\vbf}{\boldsymbol{v}}
\newcommand{\Vbf}{\boldsymbol{V}}
\newcommand{\Vcal}{\mathcal{V}}

\newcommand{\Wsf}{\boldsymbol{\mathsf{W}}}
\newcommand{\wsf}{\boldsymbol{\mathsf{w}}}
\newcommand{\wbf}{\boldsymbol{w}}
\newcommand{\Wbf}{\boldsymbol{W}}
\newcommand{\Wcal}{\mathcal{W}}

\newcommand{\xsf}{\boldsymbol{\mathsf{x}}}
\newcommand{\xbf}{\boldsymbol{x}}
\newcommand{\Xbf}{\boldsymbol{X}}
\newcommand{\Xcal}{\mathcal{X}}
\newcommand{\xch}{\check{\xbf}}
\newcommand{\xst}{\accentset{\ast}{\xbf}}
\newcommand{\Xst}{\accentset{\ast}{\Xbf}}

\newcommand{\ysf}{\boldsymbol{\mathsf{y}}}
\newcommand{\ybf}{\boldsymbol{y}}
\newcommand{\Ybf}{\boldsymbol{Y}}
\newcommand{\Ych}{\check{\Ybf}}
\newcommand{\Yst}{\accentset{\ast}{\Ybf}}
\newcommand{\Yopt}{\Ybf^{\mathrm{opt}}}

\newcommand{\zbf}{\boldsymbol{z}}
\newcommand{\Zbf}{\boldsymbol{Z}}
\newcommand{\Zsf}{\boldsymbol{\mathsf{Z}}}

\newcommand{\xibf}{\boldsymbol{\xi}}
\newcommand{\lambdabf}{\boldsymbol{\lambda}}
\newcommand{\gammabf}{\boldsymbol{\gamma}}
\newcommand{\Gammabf}{\boldsymbol{\Gamma}}
\newcommand{\mubf}{\boldsymbol{\mu}}
\newcommand{\nubf}{\boldsymbol{\nu}}
\newcommand{\taubf}{\boldsymbol{\tau}}

\newcommand{\taust}{\accentset{\ast}{\taubf}}
\newcommand{\nubfst}{\accentset{\ast}{\nubf}}
\newcommand{\nust}{\accentset{\ast}{\nu}}

\newcommand{\pibf}{\boldsymbol{\pi}}
\newcommand{\Pibf}{\boldsymbol{\Pi}}
\newcommand{\Omegabf}{\boldsymbol{\Omega}}
\newcommand{\rhobf}{\boldsymbol{\rho}}
\newcommand{\Lambdabf}{\boldsymbol{\Lambda}}
\newcommand{\Lambdast}{\accentset{\ast}{\Lambdabf}}

\newcommand{\IcI}{\Ical_{\sm{\Irm}{4}}}
\newcommand{\IcE}{\Ical_{\sm{\Erm}{4}}}
\newcommand{\IcB}{\Ical_{\sm{\Brm}{4}}}
\newcommand{\IcQ}{\Ical_{\sm{\Qrm}{4}}}
\newcommand{\IcIb}{\bar{\Ical}_{\sm{\Irm}{4}}}
\newcommand{\IcEb}{\bar{\Ical}_{\sm{\Erm}{4}}}

\newcommand{\IcBc}{\Ical_{\sm{\check{\Brm}}{5.5}}}
\newcommand{\IcBs}{\Ical_{\sm{\accentset{\ast}{\Brm}}{6}}}

\newcommand{\diagrm}{\mathrm{diag}}
\newcommand{\realrm}{\mathrm{real}}
\newcommand{\imagrm}{\mathrm{imag}}
\newcommand{\rankrm}{\mathrm{rank}}
\newcommand{\shrm}{\mathrm{sh}}
\newcommand{\maxrm}{\textnormal{max}}
\newcommand{\minrm}{\textnormal{min}}

\makeatletter
\DeclareRobustCommand{\cev}[1]{%
  \mathpalette\do@cev{#1}%
}
\newcommand{\do@cev}[2]{%
  \fix@cev{#1}{+}%
  \reflectbox{$\m@th#1\vec{\reflectbox{$\fix@cev{#1}{-}\m@th#1#2\fix@cev{#1}{+}$}}$}%
  \fix@cev{#1}{-}%
}
\newcommand{\fix@cev}[2]{%
  \ifx#1\displaystyle
    \mkern#2 1mu
  \else
    \ifx#1\textstyle
      \mkern#2 3mu
    \else
      \ifx#1\scriptstyle
        \mkern#2 2mu
      \else
        \mkern#2 2mu
      \fi
    \fi
  \fi
}
\newcommand{\cevhat}[1]{\hat{\reflectbox{\ensuremath{\vec{\ensuremath{#1}}}}}}

==> Nomenclature.tex <==
\addcontentsline{toc}{section}{Nomenclature}
\noindent
\textbf{Indices and Sets:}
\begin{IEEEdescription}[\IEEEusemathlabelsep\IEEEsetlabelwidth{${p}_{tgc}^{\mathrm{max}},{p}_{tgc}^{\mathrm{min}}$}]
    \item[$\mathcal{T}$] {Set of discrete time slots, with index $t$.}
    \item[$\Gcal$] {Set of all generators.}
	\item[$\Gcal_{t}$] {Set of all generators available at time $t\in \Tcal$.}
	\item[$\Ccal_{t}$] {Set of all contingency cases with $0\in\Ccal_{t}$ representing the base case (normal operation).}
	\item[$\Gcal_{tc}$] {Set of all generators that are available at time $t\in\Tcal$ and contingency $c\in\Ccal_{t}$, such that
		\begin{align}
			\Gcal_{t}=\cup_{c\in\Ccal_{t}}\Gcal_{tc}.\nonumber
		\end{align}}
	 \item[$\Vcal$] {Set of network buses.}
    \item[$\Ecal_{tc}$] {Set of lines at time $t\in \Tcal$ and contingency $c\in\Ccal_{t}$, such that
        \begin{align}
			\Ecal_{tc}=\Vcal \times \Vcal.\nonumber
		\end{align}}
\end{IEEEdescription}
\textbf{Parameters:}
\begin{IEEEdescription}[\IEEEusemathlabelsep\IEEEsetlabelwidth{${p}_{tgc}^{\mathrm{max}},{p}_{tgc}^{\mathrm{min}}$}]
	\item[$\alpha^{\mathrm{sqr}}_{tg}$]{Coefficient of quadratic term in cost function at time $t$ by unit $g\in\Gcal_{t}$.}
	\item[$\alpha^{\mathrm{lin}}_{tg}$]{Coefficient of linear term in cost function at time $t$ by unit $g\in\Gcal_{t}$.}
	\item[$\zeta_{tg}$]{Fixed cost coefficient at time $t$ by unit $g\in\Gcal_{t}$.}
	\item[$\eta_{tg}^{+},\eta_{tg}^{-}$]{Contingency reserves cost coefficients at time $t$ by unit $g\in\Gcal_{t}$.}
	\item[$\mu_{tg}^{+}, \mu_{tg}^{-}$]{Load-following ramping reserve cost coefficients at time $t$ by unit $g\in\Gcal_{t}$.}
	\item[$\beta_{tg}^{+}, \beta_{tg}^{-}$]{Active power re-dispatch cost coefficients at time $t$ by unit $g\in\Gcal_{t}$.}
	\item[$\kappa_{g}$]{Ramp wear and tear cost coefficients at time $t$ by unit $g\in\Gcal_{t}$.}
	\item[${p}_{tgc}^{\mathrm{max}},{p}_{tgc}^{\mathrm{min}}$] {Upper/lower limits on active power injections.}
	\item[${r}_{tg}^{\mathrm{max}},{r}_{tg}^{\mathrm{min}}$] {Upper/lower limits on reserve capacity in post-contingency dispatch quantities.}
	\item[${w}_{tg}^{\mathrm{max}},{w}_{tg}^{\mathrm{min}}$] {Upper/Lower limits on load-following reserve quantities.}
	\item[$\Delta_{g}^{\mathrm{max}},\Delta_{g}^{\mathrm{min}}$] {Upper/lower limits on transitions from base to post-contigency cases.}
	\item[$\psi_{tsc}$] {Conditional probability of contingency at time $t\in\Tcal$ and contingency $c\in\Ccal_{t}$.}
	\item[$\gamma_{t}$] {Probability of transitioning to period $t\in\Tcal$ without branching off from the central base case path to a contingency.}
\end{IEEEdescription}
\textbf{Variables:}
\begin{IEEEdescription}[\IEEEusemathlabelsep\IEEEsetlabelwidth{${p}_{tgc}^{\mathrm{max}},{p}_{tgc}^{\mathrm{min}}$}]
	\item[$p_{tgc}$] {Active power injection at time $t\in\Tcal$ by unit $g\in\Gcal_{t}$and contingency $c\in\Ccal_{t}$.}
	\item[$p^{\mathrm{ref}}_{tg}$] {Reference active power value from which generation variations are defined.}
	\item[$r^{+}_{tg},r^{-}_{tg}$] {Upward and downward contingency reserve quantities at time $t$ by unit $g\in\Gcal_{t}$.}
	\item[$w_{tg}^{+},w_{tg}^{-}$] {Upward and downward load-following ramping reserve quantities at time $t$ by unit $g\in\Gcal_{t}$.}
\end{IEEEdescription}


